Enhancing HOI Detection with Contextual Cues from Large Vision-Language Models

Human-Object Interaction (HOI) detection aims at detecting human-object pairs and predicting their interactions. However, conventional HOI detection methods often struggle to fully capture the contextual information needed to accurately identify these interactions. While large Vision-Language Models (VLMs) show promise in tasks involving human interactions, they are not tailored for HOI detection. The complexity of human behavior and the diverse contexts in which these interactions occur make it further challenging. Contextual cues, such as the participants involved, body language, and the surrounding environment, play crucial roles in predicting these interactions, especially those that are unseen or ambiguous. Moreover, large VLMs are trained on vast image and text data, enabling them to generate contextual cues that help in understanding real-world contexts, object relationships, and typical interactions. Building on this, in this paper we introduce ConCue, a novel approach for improving visual feature extraction in HOI detection. Specifically, we first design specialized prompts to utilize large VLMs to generate contextual cues within an image. To fully leverage these cues, we develop a transformer-based feature extraction module with a multi-tower architecture that integrates contextual cues into both instance and interaction detectors. Extensive experiments and analyses demonstrate the effectiveness of using these contextual cues for HOI detection. The experimental results show that integrating ConCue with existing state-of-the-art methods significantly enhances their performance on two widely used datasets.

==> sec/0_abstract.tex <==
\begin{abstract}
Human-object interaction (HOI) detection aims at detecting human-object pairs and predicting their interactions. 
However, the complexity of human behavior and the diverse contexts in which these interactions occur make it challenging. Intuitively, contextual visual cues, such as the involved participants, the body language, the surrounding environment, and the temporal period, play crucial roles in shaping these interactions. These cues are particularly vital in interpreting unseen interactions. 
In this paper, we propose three prompts with VLM to generate contextual visual cues within an image from multiple perspectives of humans. To capitalize on these rich Contextual Visual Cues, we propose a novel approach named CVC for HOI detection. Particularly, we develop a transformer-based multimodal fusion module with multitower architecture to integrate visual cue features into the instance and interaction decoders. 
Our extensive experiments and analysis validate the efficacy of leveraging the generated In this paper, we propose three prompts with VLM to generate contextual visual cues within an image from multiple perspectives of humans. To capitalize on these rich Contextual Visual Cues, we propose a novel approach named CVC for HOI detection. Particularly, we develop a transformer-based multimodal fusion module with multitower architecture to integrate visual cue features into the instance and interaction decoders.  visual cues for HOI detection. Notably, the experimental results indicate the superiority of the proposed model over the existing state-of-the-art methods on two widely used datasets. The code is available at \href{https://anonymous.4open.science/r/HCVC-B277}{https://anonymous.4open.science/r/HCVC-B277}.
\end{abstract}

%Leveraging human-centric visual cues empowers the proposed model to gain a deeper understanding of the underlying motivations in human behavior and interactions, thereby enhancing the accuracy and interpretability of interaction inferences.
%Especially, the complexity of these interactions often surpasses what can be comprehended solely through general features.

==> sec/3_Cues_extraction.tex <==
\section{Contextual Visual Cues Generation}\label{sec3}

In this section, we will introduce how to obtain contextual visual cues from VLM. It is crucial to focus on the visual cues from multiple perspectives of humans to better understand the interaction context, as human emotions and intentions often drive these interactions. To accomplish this, we propose three specialized prompts with VLM, including the participant, body language, and environmental prompt.

\begin{figure}[t]
\centering
\begin{minipage}{0.99\linewidth}\centering
\centerline{\includegraphics[height=10.9cm]{figures/framework_2.pdf}}
\end{minipage}
\vspace{0.0cm} 
\caption{\textbf{An illustration of generating contextual visual cues}, including Participant Cues, Body Language Cues, and Environmental Cues.}\label{cues}\medskip\end{figure}

\begin{figure*}[t]
\centering
\begin{minipage}{0.99\linewidth}\centering
\centerline{\includegraphics[height=6.9cm]{figures/framework.pdf}}
\end{minipage}
\vspace{-0.1cm} 
\caption{\textbf{The framework of the proposed method.} HCVC consists of two branches: one utilizes an instance decoder to detect humans and objects, while the other is dedicated to recognizing interaction using an interaction decoder. Specifically, we first employ InstructBlip to generate contextual visual cues within an image. Then, the instance and interaction decoders can be enhanced by integrating visual features and visual cue features using a multimodal fusion module.}\vspace{-0.4cm} \label{framework}\medskip\end{figure*}

\textbf{Participant Prompt.} This prompt is devised to generate visual cues focusing on humans and the objects which they potentially interact with within the image. 
Specifically, it guides VLM to pinpoint and highlight the essential humans and relevant objects in the scene. With this prompt, the generated visual cues also could provide additional insights about the participant involved in these interactions. 

The participant prompt is exemplified in Figure \ref{cues} (a). With this design, we successfully identify a girl as the main subject and enumerate several objects in her vicinity, including a tablet computer, a book, a TV, and a chair. Such detailed listing by the VLM offers a comprehensive view of the potential interaction landscape within the image, setting the groundwork for a deeper analysis of the interaction.

%\textbf{Individual fundamental prompts.} It is devised to extract fundamental individual-related details. Specifically, these prompts require the model to recognize the key individuals and objects in the image. By accurate identification of key individuals within the image, this type of prompt, denoted as $P_f$, facilitates determining who is interacting with objects. Additionally, the language model also provides information about the objects involved in these interactions and details the actions of the individuals. For example, as shown in \cref{cues} (a), the language model lists that there is a girl in the image along with some objects, including a computer, a book, a TV, and a chair.

\textbf{Body Language Prompt.} This prompt is devised to generate visual cues on human posture and facial expressions. The posture of an individual often serves as a window into their current state and intentions, while facial expressions are key indicators of emotional states. These cues are invaluable for understanding varied emotional responses to interactions across different contexts.

The body language prompt is exemplified in Figure \ref{cues} (b). The VLM discerns that the girl's legs are crossed. This detail suggests that she is sitting on the bed, as opposed to lying on it. Additionally, the visual cue inferred by the VLM indicates a relaxed demeanor, which could imply that she might be casually browsing on a laptop rather than engaging in more intensive, focused work. Such nuanced cues enhance our understanding of the scene, offering deeper insights into the nature of the interaction and the individual's engagement level.

%\textbf{Posture and expression prompts.} It concerns human pose and facial expressions, which are represented as $P_p$. Human posture can provide further insights into their state and intentions. Human expressions are instrumental in detecting their emotional states and are precious for comprehending emotional reactions within interactions and contexts. For instance, in \cref{cues} (b), the language model informs us that the girl's legs are crossed, suggesting that she is sitting on the bed rather than lying on it. The language model also suggests that the girl is in a relaxed state, implying that she might be casually browsing something on the laptop rather than actively working on it.

\textbf{Environmental Prompt.} This prompt is designed to generate visual cues related to the contextual setting surrounding individuals. The environment in which the person is situated plays a crucial role in HOI detection, as it provides essential context and background for the interactions taking place. 
The environmental cues can assist in deciphering these interactions by offering insights into the potential dynamics influenced by different settings. 
For instance, the presence of humans and dogs in a grassy outdoor area might suggest playful activities such as playing with a ball. Conversely, their presence on an indoor floor often hints at a feeding scenario. Moreover, the environmental context is instrumental in providing clues about the probable locations and characteristics of objects involved in the interaction.

The environmental prompt is exemplified in Figure \ref{cues} (c). It is determined that the girl is in a bedroom. This information suggests possible interactions with bedroom-specific objects, such as the bed, thereby enriching our understanding of the potential activities and interactions occurring in the scene.

%\textbf{Environmental prompts.} It is related to the contextual setting in which individuals are positioned. Understanding the contextual backdrop where humans are situated is particularly advantageous for the HOI task since environmental information can provide context and background for human-object interactions. Specifically, environmental prompts $P_e$ can assist in interpreting the interactions between humans and objects. Different environments can lead to distinct types of interactions. For instance, when humans and dogs are situated in a grassy area, their interaction may be playing with a ball, while their presence on an indoor floor could indicate a feeding scenario. Furthermore, the contextual setting can offer valuable hints regarding the probable object locations and characteristics. For example, in \cref{cues} (c), we learn that the girl is in a bedroom, which indicates that she may be interacting with the bed.


%After developing three perspectives of human-centric cues, we employ VLM to generate a cue set based on images. Subsequently, we use a text encoder to obtain semantic embeddings for participant cues, body language cues, and environmental cues. These embeddings, combined with visual information, will be utilized in the instance decoder and interaction decoder for instance and interaction detection.



==> sec/4_Method.tex <==
\section{HCVC}
In this paper, we propose HCVC for HOI detection, which capitalizes on human-centric visual cues extracted from large VLM. 
The framework of our approach is depicted in Figure \ref{framework}. HCVC consists of two branches: one utilizes an instance decoder~\cite{carion2020end} to detect humans and objects, while the other is dedicated to recognizing interaction using an interaction decoder. 
To harness the power of human-centric visual cues provided by VLMs, we incorporate a multimodal fusion module with a multitower architecture. This module enhances instance and interaction decoding by seamlessly integrating visual features with contextual visual cues. Detailed explanations of these components are elaborated upon in the subsequent sections.
%As introduced in~\cref{sec3}, exploring human-centric visual cues enables the model to gain deeper insights into human behavior and motivations in interactions, thereby enhancing performance and interpretability.

\subsection{Visual and Visual Cue Encoding}
%Previous approaches utilize a shared encoder for both instance detection and interaction detection, focusing solely on the visual information of images while overlooking visual cues with rich context. 

\noindent\textbf{Visual Cue Encoders.} In accordance with the content presented in Section \ref{sec3}, we devised three distinct perspectives of prompts to construct person-centric cue sets. To procure embeddings for participant cues, body language cues, and environmental cues, we specifically devised a text encoder. This encoder constitutes a stack of Transformer encoder layers. To efficiently capture intricate semantic nuances and contextual dependencies within textual data, as well as expedite model convergence, we initialized parameters using RoBERTa pretrained on vast text corpora and subsequently froze them. Furthermore, to enhance the adaptability of the RoBERTa model to our specific task, three more learnable encoder layers are added after the frozen RoBERTa. The extracted features of participant, body language, and environmental cues are denoted as $T_p$, $T_b$, and $T_e$, respectively.

%  Additionally, a text encoder is employed for the generated human-centric visual cues.
% \noindent\textbf{Visual Cue Encoder.} 
% To extract visual cue features, all obtained human-centric visual cues are fed into a text encoder. 
% In our implementation, we utilize RoBERTa \cite{liu2019roberta} as the visual cue encoder. In addition, to make the RoBERTa model more adapted to our task, three more learnable encoder layers are added after the frozen RoBERTa. 
% The extracted features of participant, body language, and environmental cues are denoted as $T_p$, $T_b$, and $T_e$, respectively.

\noindent\textbf{Visual Encoders.} 
We separately employ two different visual encoders for instance detection and interaction recognition. For instance detection, we employ a transformer framework as the image encoder~\cite{carion2020end}. Taking an image $I$ as input, we obtain visual feature $F_i$ as the input of the instance decoder. Inspired by HOICLIP \cite{ning2023hoiclip}, to improve generalization to unseen interactions, we adopt the CLIP encoder for interaction detection. Specifically, we feed the image $I$ into the CLIP encoder to obtain a feature map $F_c$, serving as the input for the subsequent interaction decoder. 

\subsection{Instance Decoder}
This section introduces the instance decoder for human and object detection. 
% The purpose of the instance decoder is to decode the visual feature into $N$ predictions.
Taking the learnable human queries $Q_h$ and object queries $Q_o$ as the input, the purpose of the instance decoder is to obtain the output for human queries $E_h\in\mathbb{R}^{N \times C_d}$ and the output of object queries $E_o\in\mathbb{R}^{N \times C_d}$ in the last decoder layer. Then, we utilize these outputs to generate $N$ predictions including human-object bounding box pairs ($B_h\in\mathbb{R}^{N \times 4}$, $B_o\in\mathbb{R}^{N \times 4}$) and object class scores $C_o\in\mathbb{R}^{N \times l_o}$, where $l_o$ is the number of object classes. Different from previous methods~\cite{TamuraOY21, LiaoZLWL022}, which solely use visual features, the HCVC instance detector utilizes features from two modalities to assist in the acquisition of $E_h$ and $E_o$: the visual features and the visual cue features. Hence, we introduce a transformer-based multimodal fusion module to ensure that the learning of $E_h$ and $E_o$ incorporates both the visual feature $F_i$ and the cue features $T$. 

\noindent\textbf{Transformer-Based Multimodal Fusion Module.}
As shown in Figure \ref{decoder},  each tower of the fusion module corresponds to the fusion of each cue feature $T \in \{T_p, T_b, T_e\}$ with the visual feature $F_i$. Take the cue feature $T_p$ as an example. We feed the queries $Q_h$ and $Q_o$ into the module, passing them through the first two attention blocks of one tower: 
\begin{equation}
[{Q}_{h}';\ {Q}_{o}'] = {\rm Cross\text{-}attn}({F}_{i}, \ {\rm Self\text{-}attn}([{Q}_{h};\ {Q}_{o}])).
\label{loss1}
\end{equation}
To incorporate cue features into the learning of $E_h$ and $E_o$, we add a new multi-head attention layer into the vanilla transformer. Then, we replace the keys (K) and values (V) with $T_p$ and feed the output into a feed-forward network. Formally, the process of obtaining the output from this tower can be described as follows:
\begin{equation}
\begin{split}
&[{E}_{h}^p;\ {E}_{o}^p] = {\rm FNN}({\rm Cross\text{-}attn}({T}_{p}, \ [{Q}_{h}';\ {Q}_{o}'])).\\
\end{split}\label{loss2}
\end{equation}
Similarly, the visual cue features $T_b$ and $T_e$ are separately fused with visual features using the other two towers of the fusion module. Finally, we aggregate the output of three towers to formulate the output $E_h$ and $E_o$. The details are provided as follows:
\begin{equation}
\begin{split}
[{E}_{h};\ {E}_{o}] = ([{E}_{h}^p;\ {E}_{o}^p] + [{E}_{h}^b;\ {E}_{o}^b] + [{E}_{h}^e;\ {E}_{o}^e])/3.
\end{split}
\label{loss3}
\end{equation}
By utilizing visual features and human-centric cue features, our instance decoder is capable of obtaining rich contextual information, leading to more resilient instance detection. %It's important to note that we do not share parameters between any of the three decoder towers, as this allows each tower to specialize in specific visual cues.

\begin{figure}[t]
\centering
\begin{minipage}{0.89\linewidth}\centering
\centerline{\includegraphics[height=7.4cm]{figures/decoder.pdf}}
\end{minipage}
\vspace{-0.1cm} 
\caption{The structure of the transformer-based multimodal fusion module with multitower architecture in the instance decoder.}\vspace{-0.4cm} \label{decoder}\medskip\end{figure}

\subsection{Interaction Decoder}
The interaction decoder is employed to predict interaction classes for the human-object pairs. Specifically, the outputs from the instance decoder, denoted as $E_h$ and $E_o$, are first pass through a projection layer to generate a set of interaction queries $Q_{inter} \in\mathbb{R}^{N \times C_i}$. 
Subsequently, we feed these queries into the interaction decoder, which also employs a transformer-based multimodal module having the same structure as this module in the instance decoder. The output of the interaction decoder is donated as $E_{inter}$. 
In detail, we replaced $[{Q}_{h};\ {Q}_{o}]$ with ${Q}_{inter}$ and ${F}_{i}$ with ${F}_{c}$ in Eq. (\ref{loss1}) and Eq. (\ref{loss2}). Note that the outputs from the three towers are concatenated instead of summed up. It is delineated as follows:
\begin{equation}
\begin{split}
{E}_{inter} = &[{E}_{inter}^p ;\  {E}_{inter}^b ;\ {E}_{inter}^e],
\end{split}
\label{loss4}
\end{equation}
where ${E}_{inter}^p$, ${E}_{inter}^b$, and ${E}_{inter}^e$ represent participant cue features, body language cue features, and environmental cue features, respectively.
% $C_i\in\mathbb{R}^{N \times l_i}$, where $l_i$ is the number of interaction classes.
% The interaction decoder decodes visual features and visual cue features into interaction category predictions $C_i$ using a similar design structure as the instance decoder. We replaced ${Q}_{ins}$ with ${Q}_{inter}$ and ${F}_{i}$ with ${F}_{c}$ in \cref{loss1}, \cref{loss2}, and \cref{loss3}. The outputs from the three decoder towers are concatenated instead of summed up.

In order to predict the interaction classes in terms of $E_{inter}$, we introduce an HOI classifier that incorporates prior knowledge using the CLIP text encoder as in previous studies~\cite{ning2023hoiclip, LiaoZLWL022}. 
The templates about HOI classes are fed into the CLIP text encoder to obtain embeddings, which are employed as the classifier's weights. 
\footnote{The template is ``a photo of a person [verb] a [object]''}
% This augmentation is particularly beneficial for handling invisible interaction classes. Specifically, each HOI category is converted into a descriptive sentence using handcrafted templates, such as ``a photo of a person [verb] a [object]'', and then these templates are fed into the CLIP text encoder to obtain embeddings of the HOI category descriptions, which are employed as the classifier's weights. 

\begin{table*}
\centering \small
\begin{tabular}{l>{\hfil}p{60pt}<{\hfil}>{\hfil}p{33pt}<{\hfil}>{\hfil}p{33pt}<{\hfil}>{\hfil}p{33pt}<{\hfil}>{\hfil}p{33pt}<{\hfil}>{\hfil}p{33pt}<{\hfil}>{\hfil}p{33pt}<{\hfil}cc} 
\toprule \multirow{3}{*}{Method} & \multirow{3}{*}{Backbone} & \multicolumn{6}{c}{ HICO-Det } & \multicolumn{2}{c}{ V-COCO } \\
\cmidrule(r){3-8}
& & \multicolumn{3}{c}{ Default } & \multicolumn{3}{c}{ Known Object } & \multirow{2}{*}{ $A P_{role}^{S1}$ }& \multirow{2}{*}{ $A P_{role}^{S2}$ }\\
\cmidrule(r){3-5} \cmidrule(r){6-8} & & Full & Rare & Non-Rare & Full & Rare & Non-Rare &   &  \\
\midrule
% \midrule \multicolumn{10}{l}{ \textbf{Two-stage methods} } \\
% VSGNet (2020) \cite{UlutanIM20}&ResNet-152& 19.80& 16.05& 20.91& -&-&-&51.8&57.0 \\
% IDN (2020) \cite{li2020hoi} & ResNet-50 & 24.58 & 20.33 & 25.86 & 27.89 & 23.64 & 29.16 & 53.3 & 60.3 \\
% SCG (2021) \cite{zhang2021spatially} & ResNet-50 & 29.26 & 24.61 & 30.65 & 32.87 & 27.89 & 34.35 & 54.2 & 60.9 \\
% UPT (2022) \cite{zhang2022efficient} & ResNet-101 & 32.62 & 28.62 & 33.81 & 36.08 & 31.41 & 37.47 & 61.3 & 67.1 \\
% \midrule \multicolumn{10}{l}{ \textbf{One-stage methods} } \\
VCL (2020) \cite{hou2020visual} & ResNet-50 & 23.63 & 17.21 & 25.55 & 25.98 & 19.12 & 28.03 & 48.3 & - \\
% PPDM (2020) \cite{LiaoLWCQF20} & Hourglass-104 & 21.73 & 13.78 & 21.40 & 24.58 & 16.65 & 26.84 & - & - \\
% HOI-Trans (2021) \cite{zou2021end} & ResNet-101 & 26.61 & 19.15 & 28.84 & 29.13 & 20.98 & 31.57 & 52.9 & - \\
ATL (2021) \cite{HouY0PT21} & ResNet-50 & 23.67 & 17.64 & 25.47 & 26.01 & 19.60 & 27.93 & - & - \\
FCL (2021) \cite{hou2021detecting} & ResNet-50 & 24.68 & 20.03 & 26.07 & 26.80 & 21.61 & 28.35 & 52.4 & - \\
% AS-Net (2021) \cite{chen2021reformulating} & ResNet-50 & 28.87 & 24.25 & 30.25 & 31.74 & 27.07 & 33.14 & 53.9 & - \\
QPIC (2021) \cite{TamuraOY21} & ResNet-101 & 29.90 & 23.92 & 31.69 & 32.38 & 26.06 & 34.27 & 58.3 & 60.7 \\
CDN (2021) \cite{zhang2021mining} & ResNet-101 & 32.07 & 27.19 & 33.53 & 34.79 & 29.48 & 36.38 & 63.9 & 65.9 \\
SSRT (2022) \cite{iftekhar2022look} & ResNet-101 & 31.34 & 24.31 & 33.32 & - & - & - & 65.0 & 67.1 \\
IF (2022) \cite{liu2022interactiveness} & ResNet-50 & 33.51 & 30.30 & 34.46 & 36.28 & 33.16 & 37.21 & 63.0 & 65.2 \\
GEN-VLKT (2022) \cite{LiaoZLWL022} & ResNet-50 &  33.75 & 29.25 & 35.10& 36.78 & 32.75 & 37.99 & 62.4 & 64.5 \\
GEN-VLKT (2022) \cite{LiaoZLWL022} & ResNet-101 & 34.95 & 31.18 & 36.08 & 38.22 & 34.36 & 39.37 & 63.6 & 65.9 \\
Zhou $et \ al.$ (2023) \cite{zhou2023learning}&  ResNet-101 & 34.42& 30.03& 35.73& 37.71& 33.74& 38.89 & 62.4& 68.1 \\
OpenCat (2023) \cite{zheng2023open}& ResNet-101& 32.68& 28.42& 33.75&-&-&-&61.9& 63.2 \\
HOICLIP (2023) \cite{ning2023hoiclip} & ResNet-50 & 34.69 & 31.12& 35.74& 37.61& 34.47& 38.54& 63.5& 64.8 \\
ADA-CM (2023) \cite{lei2023efficient}&ResNet-50 &33.80 &31.72 &34.42 &-&-&-&56.1&61.5 \\
PViC (2023) \cite{zhang2023exploring}& ResNet-50& 34.69& 32.14& 35.45& 38.14& 35.38& 38.97& 62.8& 67.8 \\
RLIPv2 (2023) \cite{yuan2023rlipv2} & ResNet-50 & 33.29 & 27.27 & 35.08 &-&-&-& 63.8 &66.4 \\
\hline \rowcolor{blue!8} $\mathrm{HCVC}_s$ & ResNet-50 & 37.22 & 36.62 & 37.40 & 39.47 & 38.43 & 39.72 & 64.1 & 66.8 \\
\rowcolor{blue!8} $\mathrm{HCVC}_l$ & ResNet-101 &  \textbf{37.54} & \textbf{37.01} & \textbf{37.78} & \textbf{39.98} & \textbf{39.01} & \textbf{40.32} & \textbf{66.0} & \textbf{68.4} \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparisons with state-of-the-art methods on the HICO-Det and V-COCO dataset.}}
\vspace{0.0cm} 
\label{regular_performance}
\end{table*}

\subsection{Training and Inference}

In the \textbf{training} phase, we employ a loss function similar to the prior transformer-based HOI methods \cite{zhang2022exploring, LiaoZLWL022}. This loss function encompasses bounding box $L1$ loss ${\mathcal{L}_{b}}$ and GIoU loss ${\mathcal{L}_{u}}$ for humans and objects, object classification loss ${\mathcal{L}_{o}}$, and interaction classification loss ${\mathcal{L}_{c}}$. The total loss is defined as follows:
\begin{equation}
{\mathcal{L}} = \lambda_b {\mathcal{L}_{b}}+\lambda_u {\mathcal{L}_{u}}+\lambda_o {\mathcal{L}_{o}}+\lambda_c {\mathcal{L}_{c}},
\end{equation}
where $\lambda_b$, $\lambda_u$, $\lambda_o$ and $\lambda_c$ are the hyper-parameters for adjusting the weights of each loss. The identical objective function is applied within the matching algorithm. Specifically, the image are fed into the HOI model to obtain $N$ predicted bounding boxes for individual and object pairs, along with their corresponding interaction categories. In the training phase, the Hungarian algorithm is employed to match ground truth with the best prediction. 
The matching cost uses the same strategy as the target cost for training backpropagation. During the \textbf{inference} phase, the confidence score of predictions is determined by adding the object score from the instance decoder and the interaction score from the interaction decoder. Subsequently, we rank the confidence scores, and the top-$k$ highest scores are considered as the final predictions. $k$ follow previous paper~\cite{kim2023relational, zhang2022exploring, dong2022category, yuan2022detecting, kim2022mstr, fang2021dirv} is set to $100$ by default.

